A Datalog Framework for Conflict-Free Replicated Data Types

Distributed applications increasingly support local-first collaboration over shared data, allowing multiple users to perform updates concurrently without global coordination. Such collaboration requires careful design to capture the intended semantics of the concurrent interactions. We introduce a declarative framework for specifying and reasoning about the semantics of conflict-free replicated data types (CRDTs) and CRDT-based applications in Datalog. The framework models CRDT semantics as executable logic programs over operation contexts, making concurrency explicit and compositional, and thus amenable to automated analysis. As one application, we use property-based testing to compare implementations. To the best of our knowledge, this is the first work to systematically use Datalog as a foundation for prototyping and analyzing complex CRDTs and their compositions. We evaluate our methodology using a collaborative graph data editing case study and report experimentation results assessing correctness validation and scalability with an increasing number of operations and replicas.

==> nested.tex <==
\section{Nested CRDTs}
\label{appendix:nested}

Our goal is to model applications that rely on both basic and derived CRDTs. Accordingly, the framework is modular: designers obtain nested data types by choosing component CRDTs and writing transformation rules from top-level events to component events. In nested structures, the decomposition is often structural. For example, a Map$\langle$Set$\rangle$  combines a set that tracks keys and a set of values for each key.


To make this example concrete, consider a Map$\langle$Set$\rangle$  with $Op_X = \{\upd{k}{v}, \rmv{k}\}$, where $v$ can be either $\add{x}$ or $\del{x}$. The first step is to define the \emph{specification level semantics} (SLS) that formalizes the behavior of the application as a single object:
%
\begin{equation}
{\footnotesize
\begin{aligned}
&\F{MapSet\_SLS}\big(\hasKV{k}{x}, (\E, \op, \vis, \ar)\big) = \text{true} \\
&\iff \exists e \in \E: \upd{k}{\add{x}} \in \op(e) \land \big( \neg \exists e' \in \E: \rmv{k} \in \op(e') \land e \xrightarrow{vis} e' \big) \\
& \quad \land \big( \neg \exists e'' \in \E: \upd{k}{\del{x}} \in \op(e'') \land e \xrightarrow{vis} e'' \big) 
\end{aligned}
}
\label{eq:mapsetadt}
\end{equation}


A Map$\langle$Set$\rangle$  contains a key \dtinline{k} and value \dtinline{x} in the set associated with \dtinline{k} if it was inserted by a \dtinline{put} operation and neither the key nor the value were later removed. 

\begin{comment}
    

\begin{equation}
\label{eq:mapSetRules}
\begin{aligned}
\mathcal{T}_{\text{keys}}(\omega) &\stackrel{\mathrm{def}}{=}
\begin{cases}
\text{add}(k) & \text{if }\omega=\text{put}(k,v),\\
\text{rmv}(k) & \text{if }\omega=\text{rmv}(k),
\end{cases}
\;\setlength{\abovedisplayskip}{4pt}
 \setlength{\belowdisplayskip}{4pt}
\mathcal{T}_{\text{vals}}(\omega) \stackrel{\mathrm{def}}{=}
\begin{cases}
\text{add}(x) & \text{if }\omega=\text{put}(k,\text{add}(x)),\\
\text{rmv}(x) & \text{if }\omega=\text{put}(k,\text{rmv}(x)).
\end{cases}\\
E_{\text{keySet}} &\stackrel{\mathrm{def}}{=} E_{\text{map}}, \qquad
E_{\text{valueSet}} \stackrel{\mathrm{def}}{=} E_{\text{map}} \setminus
\{\,e\in E_{\text{map}} \mid \exists k.\ \text{op}(e)=\text{rmv}(k)\,\}. \\
%\text{vis}_{\text{keySet}} &= \text{vis}_{\text{valueSet}} = \text{vis}_{\text{map}}, \qquad
%ar_{\text{keySet}} = ar_{\text{valueSet}} = ar_{\text{map}} .
\end{aligned}
\end{equation}

\end{comment}



\begin{comment}
\begin{equation}
\begin{aligned}
&Operations_{map} = \{\text{put}(k, v), \text{remove}(k), \text{contains}(k,x)\}\text{, where }v \in  \{\text{add}(x), \text{remove}(x)\} \\
&Operations_{keySet} = \{\text{add}(k), \text{remove}(k), \text{contains}(k)\} \\
&Operations_{valueSet} = \{\text{add}(x), \text{remove}(x), \text{contains}(x)\} \\
&\mathcal{T}_{keys}: Operations_{map} \xrightarrow{} Operations_{keySet} \\
&\mathcal{T}_{keys}(\text{put}(k,v)) = \text{add}(k)\\
&\mathcal{T}_{keys}(\text{remove}(k)) = \text{remove}(k) \\
&\mathcal{T}_{values}: Operations_{map} \xrightarrow{} Operations_{valueSet} \\
&\mathcal{T}_{values}(\text{put}(k,\text{add}(x))) = \text{add}(x)\\
&\mathcal{T}_{values}(\text{put}(k,\text{remove}(x))) = \text{remove}(x)\\
&E_{keySet} = E_{map} \\
&E_{valueSet} = E_{map} \setminus \{\, e \in E_{\text{map}} \mid \exists k.\ \text{op}(e)=\text{remove}(k) \,\}  \\
&vis_{map} = vis_{keySet} = vis_{valueSet} \\
&ar_{map} = ar_{keySet} = ar_{valueSet} \\
\end{aligned}
\label{eq:mapSetRules}
\end{equation}
\end{comment}

Next, we obtain the ICS for the Map$\langle$Set$\rangle$. Intuitively, the map contains $(k,x)$ when $k$ is present in the key set and $x$ is present in the value set associated with $k$:
%
\begin{equation}
{\footnotesize
\begin{aligned}
&\F{MapSet\_ICS}\big(\hasKV{k}{x}, (\E, \op, \vis, \ar)\big) = \text{true} \iff \\
&\quad \F{Set}\big(\hasV{k}, (\E, \op_{\keyset}, \vis, \ar)\big)
\land  \mathcal{F}_{\text{set}_k}\big(\hasV{x}, (\E_{\valset}, \op_{\valset}, \vis, \ar)\big)
\end{aligned}
}
\label{eq:mapsetics}
\end{equation}

\Cref{fig:layered_translation_mapset} presents the corresponding transformation rules.
\begin{figure}[h]
\centering
{\footnotesize
\[
\renewcommand{\arraystretch}{1.15}
\begin{array}{rcl}
\mapset.\upd{k}{\add{v}}
&\overset{\mathcal{T}}\Rightarrow&
\{\keyset.\add{k}, \valset.\add{v}\} \\

\mapset.\upd{k}{\del{v}}
&\overset{\mathcal{T}}\Rightarrow&
\{\keyset.\add{k}, \valset.\del{v}\} \\

\mapset.\rmv{k}
&\overset{\mathcal{T}}\Rightarrow& \{ \keyset.\del{k} \} 
\end{array}
\]
}
\caption{Layered transformation for update-wins Map$\langle$Set$\rangle$.}
\label{fig:layered_translation_mapset}
\end{figure}




In Datalog, the event facts of the Map$\langle$Set$\rangle$ \dtinline{mapSetOp(E,Op,InnerOp,K,X)} consist of the event identifier \dtinline{E}, the map-level operation \dtinline{Op}, the inner set operation \dtinline{InnerOp} and the operation parameters \dtinline{K} and \dtinline{X} (Listing \ref{lst:mapset}). \dtinline{keysOp} and \dtinline{setOp} correspond to the transformation rules. \dtinline{mapState} computes the final state. Note that a key might exist with an empty value set. For that we use the empty value \dtinline{""}. 


\begin{lstlisting}[style=souffleStyle, caption = Map$\langle$Set$\rangle$  semantics expressed in Datalog., label = lst:mapset]
keysEvent(E, "add", K) :- mapSetEvent(E, "upd",  _, K, _).
keysEvent(E, "del", K) :- mapSetEvent(E, "rmv", _, K, _).
setEvent(E, InnerOp, X, K) :- mapSetOp(E, "upd", InnerOp, K, X), not postVisRemove(E).
mapState(K, X)  :- keysState(K), setState(K, X).
mapState(K, "") :- keysState(K), not setState(K, _).
\end{lstlisting}

Soufflé does not support dynamic instantiation of modules at runtime. In particular, a Map$\langle$Set$\rangle$ cannot allocate a fresh set instance per key during evaluation. We therefore encode all inner sets within a single indexed set instance, using an additional identifier (the key) to distinguish per-key state. The corresponding code can be found in \Cref{lst:valueset}.

\begin{lstlisting}[style=souffleStyle, caption = Value set semantics expressed for ICS Map$\langle$Set$\rangle$., label = lst:valueset]
laterVisOpSet(E1, P) :- setEvent(E1, _, X, S), setEvent(E2, "del", X, S), 
                        visible(E1, E2), E1\=E2.
lastVisibleOpSet(E1) :- setEvent(E1, _, _, _), not laterVisOpSet(E1, E2).
setState(S, X)       :- setEvent(E, "add", X, S), lastVisibleOpSet(E).
\end{lstlisting} 


With this encoding pattern, deeper nesting (e.g. maps of maps) reduces to the repeated use of transformation rules and identifiers.

